Worst-Case Risk Quantification under Distributional Ambiguity using Kernel Mean Embedding in Moment Problem

In order to anticipate rare and impactful events, we propose to quantify the worst-case risk under distributional ambiguity using a recent development in kernel methods -- the kernel mean embedding. Specifically, we formulate the generalized moment problem whose ambiguity set (i.e., the moment constraint) is described by constraints in the associated reproducing kernel Hilbert space in a nonparametric manner. We then present the tractable approximation and its theoretical justification. As a concrete application, we numerically test the proposed method in characterizing the worst-case constraint violation probability in the context of a constrained stochastic control system.

==> draft/pf_conv_ambi.tex <==
Let $P_1, P_2\in \mathcal C$, and let  $P = t P_1+(1-t)P_2$, where $t\in[0,1]$. It suffices to show $P\in\mathcal C$ for any choices of $P_1, P_2, t$. Let $\mu_P = \int\phi(x)dP(x)$, we have
\begin{multline}
 \|\mu_P - \hat\mu\|_\rkhs= \|t\mu_{P_1} - t\hat\mu +(1-t)\mu_{P_2} - (1-t)\hat\mu\|_\rkhs\\
 \leq \|t\mu_{P_1} - t\hat\mu \|_\rkhs+\|(1-t)\mu_{P_2} - (1-t)\hat\mu\|_\rkhs\\
 \leq t\epsilon + (1-t)\epsilon = \epsilon.
 \end{multline}
Hence, $P\in\mathcal C$.



==> draft/thm_conic.tex <==
We first derive the conic dual of the KME-MP in the following results.

\begin{prop}
(Conic duality of KME-MP)
The optimal value of the KME-MP is equivalent to the following conic optimization problem.


$$
\begin{aligned}
&\mxz_{y} & &  \pip{y}{\hat P} - \epsilon\hnorm{y} \\
&\sjt& & l-y\in K^*, y\in\rkhs
\end{aligned}
\label{eq:conic_dual}
$$

where $\mathcal H$ is the RKHS in the primal problem,  $K^*$ is the dual cone of $\mathrm{cone}(\mathcal P)$. 
$$
K^*:= \{h\mid\int h(x)dP\geq0, \forall P \in \mathrm{cone}(\mathcal P), h \text{ is measurable}\}
$$
Furthermore, the primal problem is strictly feasible and strong duality holds.

\end{prop}

The proof is given in the appendix. Then, we use a standard results in the literature.

\begin{definition}

(Choquet representation)
We say a set of distributions $\mathcal Q$ is generated by $\mathbb T$ if
$$
\exists m \in {\mathcal P}(\mathbb T) \mid Q (\cdot) = \int_{\mathbb T} e(\cdot) d m (e), \forall Q\in {\mathcal Q}.
$$
$m$ is the called mixture distribution.

\end{definition}

We use $\mathrm{mix}(\mathbb T)$ to denote the mixture hull of the generating set $\mathbb T$. 
$$
\mathrm{cone}(\mathcal P) \subseteq \mathrm{mix}(\mathbb T)
$$
The following result is due to the modern proof of \cite{shapiroDualityTheoryConic2001} as well as the classical results from \cite{rogosinskiMomentsNonNegativeMass}.

\begin{lemma}

The conic dual problem is equivalent to the following,
$$
\begin{aligned}
&\mxz_{y} & &  \pip{y}{\hat P} - \epsilon\hnorm{y} \\
&\sjt& & \int l(x)-y(x)\ d\tau(x)\geq0,\ \forall\tau\in \mathbb T,\\
&&&y\in\rkhs
\end{aligned}
\label{eq:conic_dual_finite}
$$
where $\mathbb T$ is the set of distriubitons supported on $N$  points,
$$
\mathbb T := \{P\mid P = \sum_{i=1}^N{\alpha_i}\delta_{x_i}, \sum_{i=1}^N\alpha_i =1,
\alpha_i\geq0, i=1\dots N, x_i\in\mathbb R^n\}.
$$

\end{lemma}

This is, of course, a semi-infinite program. However, if we take the dual again, we will obtain the same primal problem, but with $\mathcal P$ replaced by $\mathbb T$ , which indicates that it suffices to look for solutions in the class of distributions $\mathbb T$. This is summed up as following.

\begin{theorem}

For the KME-MP problem, it suffices to consider discrete distributions that are supported on $N$  points, i.e.,
$$
\begin{aligned}&\underset{P,\mu}{\mnz} &  & \int l(x) \ dP(x) \\
&\sjt& & \|\mu - \mu_{\hat P}\|_\rkhs\leq \epsilon\\
&&&     \int \phi(x) \ dP(x) = \mu\\
&&& P\in \mathbb T, \mu\in \rkhs,
\end{aligned}
$$
where $\mathbb T$ is the set of distriubitons supported on $N$  points,
$$
\mathbb T := \{P\mid P = \sum_{i=1}^N{\alpha_i}\delta_{x_i}, \sum_{i=1}^N\alpha_i =1,
\alpha_i\geq0, i=1\dots N, x_i\in\mathbb R^n\}.
$$
\end{theorem}
The implication of our theretical analysis is that, we only need to focus our attention on discrete distributions supported on $N$ points, i.e.
\[
p^* = \sum^{N}_{i=1} \alpha_i \delta_{x_i}, \text{ for some }x_i\in \mathbb{R}^n.
\]


